Algorithms for Sparse LPN and LSPN Against Low-noise

We consider sparse variants of the classical Learning Parities with random Noise (LPN) problem. Our main contribution is a new algorithmic framework that provides learning algorithms against low-noise for both Learning Sparse Parities (LSPN) problem and sparse LPN problem. Different from previous approaches for LSPN and sparse LPN, this framework has a simple structure and runs in polynomial space. Let $n$ be the dimension, $k$ denote the sparsity, and $\eta$ be the noise rate. As a fundamental problem in computational learning theory, Learning Sparse Parities with Noise (LSPN) assumes the hidden parity is $k$-sparse. While a simple enumeration algorithm takes ${n \choose k}=O(n/k)^k$ time, previously known results stills need ${n \choose k/2} = \Omega(n/k)^{k/2}$ time for any noise rate $\eta$. Our framework provides a LSPN algorithm runs in time $O(\eta \cdot n/k)^k$ for any noise rate $\eta$, which improves the state-of-the-art of LSPN whenever $\eta \in ( k/n,\sqrt{k/n})$. The sparse LPN problem is closely related to the classical problem of refuting random $k$-CSP and has been widely used in cryptography as the hardness assumption. Different from the standard LPN, it samples random $k$-sparse vectors. Because the number of $k$-sparse vectors is ${n \choose k}<n^k$, sparse LPN has learning algorithms in polynomial time when $m>n^{k/2}$. However, much less is known about learning algorithms for constant $k$ like 3 and $m<n^{k/2}$ samples, except the Gaussian elimination algorithm of time $e^{\eta n}$. Our framework provides a learning algorithm in $e^{O(\eta \cdot n^{\frac{\delta+1}{2}})}$ time given $\delta \in (0,1)$ and $m \approx n^{1+(1-\delta)\cdot \frac{k-1}{2}}$ samples. This improves previous learning algorithms. For example, in the classical setting of $k=3$ and $m=n^{1.4}$, our algorithm would be faster than than previous approaches for any $\eta<n^{-0.7}$.

==> generalization_p.tex <==
\subsection{Generalization to $\mathbf{F}_p$} 
\textcolor{red}{use $\mathbf{F}_p$ instead of $\mathbf{F}_q$...no need to write all details, but show  new parameters and necessary calculations}
Similarly, we need to calculate the number of random vectors in $\mathbf{F}_p^n$ span the whole space.

New definition: with probability $\eta$, label is a random element in $F_p$ not $F_p^*$ 

\begin{proposition}\label{lem:ksparse_p_span}
     For any odd number $k<n/\log n$, $t=c_2\max\{\frac{n\ln n }{k},10\log_{p-1}n+n\log_{p-1}p\}$random $k$-sparse vectors in $\mathbf{F}_p^n$ span the whole space $\mathbb{F}_p^{n}$ with probability $1-1/n^5$ (for some constant $c_1$).
\end{proposition}
\begin{proofof}{Proposition~\ref{lem:ksparse_p_span}}
    Similarly, we consider the dual vector for a given linear subspace $U$ of dimension $n-1$.
    We need to calculate \textcolor{red}{Do not understand this calculation!!!!!}
    Note that
\begin{align*}
    \Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0]&=\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0|x\cap v=0]\Pr[x\cap v=0]+\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0|x\cap v>1]\Pr[x\cap v>1]
\end{align*}


    
    \begin{align*}
        \Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0]&\leq\frac{\binom{n-\ell}{k}(p-1)^{k}}{\binom{n}{k}(p-1)^k}+\sum_{2\leq i\leq \min\{\ell,k\}}\frac{\binom{\ell}{i}\cdot\binom{n-\ell}{k-i}(p-1)^{i-1}(p-1)^{k-i}}{\binom{n}{k}(p-1)^k}\\
        &= \frac{\binom{n-\ell}{k}}{\binom{n}{k}}+\left(1-\frac{\binom{\ell}{1}\binom{n-\ell}{k-1}}{\binom{n}{k}}-\frac{\binom{n-\ell}{k}}{\binom{n}{k}}\right)\cdot\frac{1}{p-1}\\
        &=\frac{\binom{n-\ell}{k}}{\binom{n}{k}}+\left(1-(1+\frac{\ell k}{n-\ell-k+1})\frac{\binom{n-\ell}{k}}{\binom{n}{k}}\right)\cdot \frac{1}{p-1}\\
      &=\frac{1}{p-1}+\left(\frac{p-2}{p-1}-\frac{\ell k}{(n-\ell-k+1)(p-1)}\right)\frac{\binom{n-\ell}{k} }{\binom{n}{k}} .
      % &\leq \frac{1}{p-1}+\left(\frac{p-2}{p-1}-\frac{\ell k}{(n-\ell-k+1)(p-1)}\right)e^{-\frac{k\ell}{n}}.
    \end{align*}
    \begin{itemize}
        \item for $\ell\leq \frac{8n}{k}$, 
        we have $\frac{\binom{\ell}{1}\binom{n-\ell}{k-1}}{\binom{n}{k}}=\Omega(\frac{k\ell}{n})$.
let $i_1,....,i_{\ell}$ be $\ell$ positions that $v_{i_k}\neq 0$. There are $(p-1)^{\ell}$ such $v$.
        $$\Pr_{ x\sim \binom{n}{k}\cdot (p-1)^k}[\forall v \text{ satisfies } v_{i_1}\neq 0,....,v_{i_{\ell}}\neq 0,\langle x,v\rangle\neq 0]\geq \frac{\binom{\ell}{1}\binom{n-\ell}{k-1}}{\binom{n}{k}}=\Omega\left(\frac{k\ell}{n}\right)$$
        Thus 
        $$ \Pr_{ x\sim \binom{n}{k}\cdot (p-1)^k}[\exists v \text{ satisfies } v_{i_1}\neq 0,....,v_{i_{\ell}}\neq 0,\langle x,v\rangle= 0]\leq \left(1-\Omega\left(\frac{k\ell}{n}\right)\right).$$
 
        \item for $\ell\geq \frac{8n}{k} $, $$\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\exists v \text{ satisfies } v_{i_1}\neq 0,....,v_{i_{\ell}}\neq 0,\langle x,v\rangle= 0]\leq e^{-8}+\frac{1}{p-1}.$$
        \wxnote{this is not right. How can we prove $$\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\exists v \text{ satisfies } v_{i_1}\neq 0,....,v_{i_{\ell}}\neq 0,\langle x,v\rangle= 0]\leq O(1).$$}
        \end{itemize}
Note that the term $e^{-8}$ is commonly used by $(p-1)^{\ell}$ terms. 
Finally, we apply a union bound over all linear subspaces of dimension $(n-1)$.

Consider for $\ell>\frac{8n}{k}$,

Since $x\cap v$ satisfies the hypergeometric distribution.
$\E[|x\cap v|]=\frac{k\ell}{n}$ and $\Var(|x\cap v|)=\frac{k\ell}{n}\frac{(n-k)(n-\ell)}{n(n-1)}$.
Let $Z=|x\cap v|$.
By Chebyshev's inequality,
$$\Pr[|Z-\E[Z]|\geq 2\sqrt{\frac{k\ell}{n}}]\leq \frac{1}{4}.$$

For $\ell>\frac{8n}{k}$, $\Pr[|x\cap v|\geq 2]>\frac{3}{4}.$
Then by the chernoff bound, with probability $1-e^{-\frac{t}{8}}$, there are at least $\frac{t}{2}$ random $k$-sparse vectors intersect with $v$ for at least $2$ positions. Here we union bound on all $S\sim \binom{n}{\ell}$. Thus with probability at least $1-2^ne^{-\frac{t}{8}}$, there are at least $\frac{t}{2}$ random $k$-sparse vectors intersect with $v$ for at least 2 positions.

In this case, 
$\Pr[\langle x,v\rangle=0]\leq \frac{1}{p-1}$. 
Thus 
\begin{align*}
    &\Pr\left[\text{$t$ random $k$-sparse vectors } \bot~v,|v|=\ell\right]\\
    &\leq (\frac{1}{p-1})^{\frac{t}{2}}.
\end{align*}



\begin{align*}
&\Pr[dimension(\text{$t$ random $k$-sparse vectors})\le n-1] \\
=& \sum_{\ell=1 }^{n} \Pr\left[\exists v,\text{$t$ random $k$-sparse vectors } \bot~v,|v|=\ell\right]\\
=& \sum_{\ell\leq \frac{8n}{k}} \Pr\left[\exists v,\text{$t$ random $k$-sparse vectors } \bot~v,|v|=\ell\right]+\\
&\sum_{\ell> \frac{8n}{k}} \Pr\left[\exists v,\text{$t$ random $k$-sparse vectors } \bot~v,|v|=\ell\right]\\
&\leq \sum_{\ell \leq \frac{8n}{k}}\sum_{S\in \binom{[n]}{\ell}} \Pr\left[\exists v,\text{$t$ random $k$-sparse vectors } \bot~v,v_i\neq 0\,\, i\in S\right] \\
&+ \sum_{v:|v| > \frac{8n}{k}}\Pr\left[\text{$t$ random $k$-sparse vectors } \bot~v\right] \\
& \leq \sum_{\ell\leq \frac{8n}{k}} {n \choose \ell}e^{-\frac{k\ell t}{n}} +p^n(\frac{1}{p-1})^{\frac{t}{2}}+2^ne^{-\frac{t}{8}} .
\end{align*}


When $t\geq 10\frac{n\ln n }{k}$, the term in the first summation $${n \choose \ell}e^{-\frac{k \ell \cdot t}{n}}<n^{\ell} e^{-\frac{\ell k t}{n}}<n^{-10\ell}.$$
For the last term, we need $p^{n}\left(\frac{1}{p-1}\right)^{\frac{t}{2}}\leq n^{-10}.$ This means $t\geq 2(10\log_{p-1} n+n\log_{p-1}p).$
Hence for $t=c_2\max\{\frac{n\ln n }{k},10\log_{p-1} n+n\log_{p-1}p\}$ ,$\Pr[dimension(\text{$t$ random $k$-sparse vectors})\le n-1] \le n^{-5}$ .
% \begin{itemize}
%     \item 
%     If $\ell<k$, $\sum_{2\leq i\leq \min\{\ell,k\}}(p-1)^{i-k}\leq \frac{1}{p-2}.$ So the probability $\leq \frac{1}{p-2}$

%     \item $\ell<\frac{8n}{k}$, $\frac{\binom{\ell}{1}\binom{n-\ell}{k-1}}{\binom{n}{k}}\geq \frac{\ell\cdot k}{n}e^{-8}]\leq (1-\frac{\ell\cdot k}{n}e^{-8})\sum_{2\leq i\leq \min\{\ell,k\}}(p-1)^{i-k}.$ Similarly, we still have $\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0]\leq 1-\Omega(\frac{k\ell}{n}).$
%     \item $\ell>\frac{8n}{k}$, $\Pr_{x\sim \binom{n}{k}\cdot (p-1)^k}[\langle x,v\rangle=0]\leq \sum_{i\in [\frac{k \ell}{n}- 2 \sqrt{\frac{k \ell}{n}},\frac{k \ell}{n} + 2 \sqrt{\frac{k \ell}{n}}]}(p-1)^{i-k}+\frac{1}{4}\leq 2(p-1)^{\frac{k\ell}{n}+2\sqrt{\frac{k\ell}{n}}-k}+\frac{1}{4}$

%     $(\sqrt{\frac{k\ell}{n}}+1)^2-k-1<0\Rightarrow \ell<\frac{n(k-2\sqrt{k+1})}{k}$
%     \item $\ell\geq \frac{n(k-2\sqrt{k+1})}{k}$
% \end{itemize}
   

\end{proofof}
\begin{corollary}{\label{cor:p-verification}}
    For the $(k,\eta)$-LSPN problem of dimension $n$, $m= \frac{8(n\ln p+5\ln n)}{(1-\frac{1-2\eta}{p-2})^2}$ random samples guarantee that with probability $1-1/n^5$, $\secret$ is the only vector $v$ in $\mathbf{F}_p^n$ satisfying
    $\sum_{i=1}^m \mathbf{1}(\langle x_i,v\rangle \neq y_i) \le (\eta + c_0 \cdot \frac{k}{n}) \cdot m$ (for some constant $c_0$).
\end{corollary}
\begin{proofof}{Corollary~\ref{cor:p-verification}}
Similarly, we consider 
$$\Pr_x[\langle x,\textbf{secret}-v \rangle\neq 0].$$
Let $\ell=|\textbf{secret}-v|$.
\begin{itemize}
    \item for $\ell<\frac{8n}{k}$, let $S\sim \binom{[n]}{\ell}$ $$\Pr_x[(\textbf{secret}-v)_i\neq 0,\, i\in S,\langle x,\textbf{secret}-v \rangle\neq 0]=\Omega(\frac{\ell\cdot k}{n}).$$
    \item for $\ell\geq \frac{8n}{k}$, let $Z=x\cap (\secret-v)$
    $\Pr[|Z|\geq 2]>\frac{3}{4}$. Then by the chernoff bound, with probability $1-2^ne^{-\frac{m}{8}}$, there are at least $\frac{m}{2}$ random $k$-sparse vectors intersecting with all $v$ for at least 2 positions. In this case $\Pr[\langle x,\secret-v\rangle\neq 0]=\Omega(\frac{p-2}{p-1}).$
\end{itemize}
Then, we set the threshold $m(\eta+c_3\cdot \frac{k}{n})$ for a sufficiently small constant $c_3$ to distinguish \textbf{secret} from the rest hypotheses $v\in \mathbf{F}_p^n\backslash\{\textbf{secret}\}$.
Now we bound the probability that $m_{\secret}<m(\eta + c_0 \cdot \frac{k}{n})$ and $m_v \ge (\eta + c_0 \cdot \frac{k}{n})$ for any $v \neq \secret$.
for $\ell<\frac{8n}{k}$, let $S\sim \binom{[n]}{\ell}$ 

We want to compute 
\begin{align*}
    &\Pr\left[\exists v \textit{ satisfying } v-\secret\neq 0, m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\
&=\sum_{\ell=1}^n\Pr\left[\exists v \textit{ satisfying } |v-\secret|=\ell , m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\
&=\sum_{\ell\leq \frac{8n}{k}}\Pr\left[\exists v \textit{ satisfying } |v-\secret|=\ell , m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\
&+\sum_{\ell> \frac{8n}{k}}\Pr\left[\exists v \textit{ satisfying } |v-\secret|=\ell , m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\
&\leq \sum_{\ell\leq \frac{8n}{k}}\sum_{S\in \binom{[n]}{\ell}}\Pr\left[\exists v \textit{ satisfying } v_i-\secret_i\neq 0,i\in S , m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\
&+\sum_{v:|v|\geq \frac{8n}{k}}\Pr\left[  m_v<m(\eta+c_3\cdot \frac{k}{n})\right]
\end{align*}


\begin{align*}
   &\Pr\left[\exists v \textit{ satisfying } v_i-\secret_i\neq 0,i\in S , m_v<m(\eta+c_3\cdot \frac{k}{n})\right] \\
   &=\Pr[\min_{v:v_i-\secret_i\neq 0,i\in S} m_v<m(\eta+c_3\cdot \frac{k}{n})]
\end{align*}

\begin{align*}
    \min_{v:v_i-\secret_i\neq 0,i\in S}m_v&=\min_{v:v_i\neq 0,i\in S}\sum_{j=1}^m\mathbf{1}(y_j\neq \langle x_j,v\rangle)\\
    &\geq \sum_{j=1}^m\min_{v:v_i-\secret_i\neq 0,i\in S}\mathbf{1}(y_j\neq \langle x_j,v\rangle)\\
    &=\sum_{j=1}^m\mathbf{1}(\forall v:v_i-\secret_i\neq 0,i\in S, y_j\neq\langle x_j,v\rangle )\\
\end{align*}
Let $m'_v=\sum_{j=1}^m\mathbf{1}(\forall v:v_i-\secret_i\neq 0,i\in S, y_j\neq\langle x_j,v\rangle ).$
However 
\begin{align*}
    &\E[\mathbf{1}(\forall v:v_i-\secret_i\neq 0,i\in S, y_j\neq\langle x_j,v\rangle )]\\
    &=\eta +(1-2\eta)\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]
\end{align*}

With a similar argument
\begin{align*}
    &\Pr\left[ \min_{v:v_i-\secret_i\neq 0,i\in S} m_v<m(\eta+c_3\cdot \frac{k}{n})\right]\\ 
    &\leq \Pr[m'_v<m(\eta+c_3\cdot \frac{k}{n})]\\
    & = \Pr\left[ m'_v< \frac{\eta  + c_0 \cdot \frac{k}{n}}{\eta  + (1-2\eta) \cdot \Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]} \cdot \E[m'_v] \right]\\
    &\leq e^{-\frac{\E[m'_v]\cdot \min\{\frac{\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]}{4\eta},\frac{1}{4}\}^2}{2}}.
\end{align*}
 For convenience, let $\ell := |\secret-v|$ and $s_2$ be the largest index of $\ell$ such that $\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]\le \eta$ for any $|\secret-v| \le s_2$. Since $\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]=\Theta(\ell k/n)$ when $\ell k<n$, $s_2 = \Theta(\eta n/k)$.
\begin{itemize}
    \item $\ell<s_2$: $\\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]=\Omega(\frac{\ell\cdot k}{n})$ and $\Pr[m'_v<m(\eta+c_1\cdot \frac{k}{n})]\leq e^{-\Omega(m\cdot\frac{\ell^2k^2}{n^2\eta})}$ in this case. We need $m=\Omega(\frac{\eta n^2\cdot \log n}{k^2})$ such that their union bound is at most $n^{-10}$.
    \item $\ell\in(s_2,\frac{8n}{k})$:$\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]=\Omega(\frac{\ell\cdot k}{n})>\eta$ and $\Pr[m'_v<m(\eta+c_1\cdot \frac{k}{n})]\leq e^{-\Omega(m\cdot\frac{\ell k}{n})}$
    Since the number of such $v$'s is ${n \choose \ell}\le n^\ell$, we need $m = \Omega(\frac{n \log n}{k})$ such that their union bound is at most $n^{-10}$.
    \item $\Pr[\forall v:v_i-\secret_i\neq 0,i\in S,\langle x_j,\secret\rangle\neq \langle x_j,v\rangle]=\Omega(1)$\wxnote{I am not sure about this unless we can prove } and $\Pr[m'_v<m(\eta  + c_0 \cdot \frac{k}{n})] \le e^{-\Omega(m)}$. \wxnote{Here we still needs $p^n$ terms.}Since the number of such $v$'s is at most $2^n$, we need $m=\Omega(n)$ for the union bound.
    
\end{itemize}
\end{proofof}


\iffalse
\begin{algorithm}[H]
    \caption{Main Procedure}
    \label{alg::sparseLPN_p}
    \begin{algorithmic}[1]
        \Function{PartialLearn}{$I\subset [n],m,\mX \in \mathbf{F}_p^{m \times I},\by \in \mathbf{F}_p^m$} \qquad \Comment the goal is to partially learn $\secret(I)$ given $m$ samples $(x_i,y_i)$ in $(\mX,\by)$ whose $supp(x_i) \subset I$
        \State $q \gets |I|$
        \State $C \gets $ a sufficiently large constant
        
        \If {$m<C \cdot q \cdot \max\{1,\frac{\log q}{k(p-1)}, \frac{\eta q \log q}{(p-1)^2k^2}\}$}
               \State \Return $\bot$
        \EndIf
        \State $d \gets c_1 \cdot q \cdot \max\{1,\frac{\log q}{(p-1)k}\}$ is the number of required samples from Proposition~\ref{lem:ksparse_span} 
        \State $m' \gets 100 \cdot d$ \qquad \Comment{Use the first $m'$ samples to try Gaussian eliminations and the rest $(m-m')$ samples for verification}

        \State $L \gets 10 q^2 + 10 \log q \cdot e^{\frac{200c_1}{99} \cdot \eta q \max\{1,\frac{\log q}{(p-1)k}\}}$ \Comment{Number of rounds of Gaussian elimination}
        
        \For{$i=1,\ldots,L$}
            \State Pick a random set of samples: $T \sim {[m'] \choose d}$ 
            \If{rank$\{\bx(T,I)\}=q$} \Comment{Recall $q:=|I|$}
                \State Apply Gaussian elimination to find $ans\in \mathbf{F}_2^I$ such that
                    $$\mX(T,I) \cdot ans = y(T)$$
                \State Count $s \gets \sum_{i=m'+1}^m \mathbf{1}\big( \langle x_i, ans \rangle \neq y_i \big)$ 
                \If{$s \le (m-m')\cdot (\eta + c_0 \cdot \frac{k}{q})$}             \Comment{$c_0$ is the constant in Corollary~\ref{cor:verification}}
                    \State \Return $ans$
                \EndIf 
            \EndIf
        \EndFor
        \State Return $\bot$        
        \EndFunction
        \Function{Learn}{$k,\eta,\delta$}               
       
        \State $t \gets n^{\frac{1-\delta}{2}}$ and $q \gets n/t$ 

        \State $m \gets O(q) \cdot \max\{1,\frac{\log q}{(p-1)k}, \frac{\eta q \log q}{(p-1)^2k^2}\} \cdot (et)^k$ \Comment{Number of samples}

        \State define $t$ intervals $I_1,\ldots, I_t \subset [n]$: $I_j \gets \{(j-1)\cdot q + 1, \ldots, j \cdot q\}$ for each $j \in [t]$
        
        \State initialize $m_j =0$ and  matrix $\mX_j \in \mathbf{F}_2^{m_j \times n}$ and $\by_j \in \mathbf{F}_2^{m_j}$ for each $j \in [t]$
        
        \For {$i= 1,2,\ldots, m$}   \Comment{Allocate $m$ samples according to these intervals}
            \State Take a fresh sample $(x,y)$
            \If{$supp(x) \subset I_j$ for some interval $I_j$}
                \State $m_j \gets m_j +1$
                \State $\mX_j(m_j,\cdot) \gets x$ and $\by_j(m_j)=y$
            \EndIf
        \EndFor
        \For {$j=1,\ldots,t$}
            \State $\secret(I_j) \gets \textsc{PartialLearn}(I_j,m_j,\mX_j, \by_j)$
        \EndFor
        \State \Return $\secret$                
        \EndFunction
    \end{algorithmic}
\end{algorithm}






\begin{itemize}
    \item For $1\le|d|\le 100\frac{n}{k}$,  $\Omega (1)\le\Pr[2\mid x\cdot d]\le 1-\Omega(\frac{k|d|}{n})$.\wxnote{A little weird since $\frac{k|d|}{n}\leq 100$ and $\Omega(\frac{k|d|}{n})$}
\begin{align*}
\Pr[x\cdot d=0]&={n-k\choose |d|}/{n\choose |d|}\cr
&= \Omega(1)\cr
\Pr[x\cdot d=1]&= k {n-k\choose|d|-1}/{n-k\choose |d|}\cdot{n-k\choose |d|}/{n\choose|d|}\cr
&\ge \frac{k |d|}{n-k-|d|+1}\cdot(\frac{n-k-|d|}{n-|d|})^{|d|}\cr
&= \Omega(\frac{k|d|}{n})
\end{align*}

Note that the former equation also holds for $|d|=0$;

    \item For $100 \frac{n}{k}<|d|\le \frac{n}{2}$, $\Omega(1) \le\Pr[2\mid x\cdot d]\le 1-\Omega(1)$. 
    $$
            \Pr[x\cdot d=i]=\binom{k}{i}\binom{n-k}{|d|-i}/{n\choose |d|}
    $$
    For simplicity, let $p=\frac{k}{n}$.\wxnote{Do we really need 100 here?}
By Chebyshev's bound:    
\begin{align*}
    \Var[x\cdot d]=|d|p(1-p)(1-\frac{|d|-1}{n-1})&\le |d|p\cr
    \Pr[|x\cdot d-p|d||\ge2\sqrt{p|d|} ]&\le \frac{1}{4}
\end{align*}



 %   $ = h(k,n,|d|,i)$ where $h$ represent the Hypergeometric distribution.


    We choose $l, r$ such that $r\ge 1+2/\sqrt{p|d|},l\le 1-2/\sqrt{p|d|}$, and $2\mid rp|d|,2\nmid lp|d|$ are both integers. Since $p|d|\ge 100$, there exist such $l,r$ satisfyng $0.5\le l< r\le 1.5$. Then, we can bound the ratio of probability between adjacent $i$s.

    $$\text{Ratio}(i):=\frac{\binom{k}{i}\binom{n-k}{|d|-i}}{\binom{k}{i+1}\binom{n-k}{|d|-i-1}}=\frac{(i+1)(n-k-|d|+i+1)}{(k-i)(|d|-i)}.$$
\znote{the denominator is problematic when d is close to $n$, we need another case}


        The above probability increases monotonically with respect to $i$. Therefore, when $i\in [lp|d|+1,rp|d|-1]$, the ratio can be upper bounded by (without loss of generality, assume $p\le 0.5$):
\begin{align*}
    \text{Ratio}(i)&\le\frac{rp|d|(n-|d|-k+rp|d|)}{(k-rp|d|+1)(|d|-rp|d|+1)}\cr
    &\le\frac{1.5p|d|n}{0.25k \cdot 0.25|d|} \le 24
\end{align*}

It can be lower bounded by:
\begin{align*}
    \text{Ratio}(i)&\ge\frac{lp|d|(n-|d|-k+lp|d|)}{(k-lp|d|)(|d|-lp|d|)}\cr
    &\ge\frac{lp(n-|d|-k+lp|d|)}{k }\cr
    &=l(1-\frac{|d|}{n}-p+lp\frac{|d|}{n})\cr
    &\ge l(1-0.5-0.5+0.5^3)=\frac{1}{16}\tag{minimized when |d|/n=p=0.5}
\end{align*}
Thus 
\begin{align*}
    \Pr[2|x\cdot d]&=\sum_{2|i}{\Pr[x\cdot d=i]}\\
    &=\sum_{2|i,i\in [lp|d|+1,rp|d|-1]}{\Pr[x\cdot d=i]}+\sum_{2|i,i\not\in [lp|d|,rp|d|]}{\Pr[x\cdot d=i]}\\
    &\leq \frac{1}{1+\frac{1}{24}}(1-\Pr\left[lp|d|> x\cdot d\text{ or }x\cdot d<rp|d|\right])+\Pr[lp|d|\leq x\cdot d\leq rp|d|]\\
    &\leq \frac{24}{25}+\frac{1}{25}\cdot \frac{1}{4}=0.97
\end{align*}


    \item if $n\ge |d|>\frac{n}{2}$, $\Pr[2|x\cdot d=0]\le constant$.\wxnote{We need to avoid the case $|d|=n$. We need to constant to be less than 1.}

    The probability is symmetric with respect to $|d|$, that is: $h(k,n,|d|,i)=h(k,n,n-|d|,k-i)$ were $h$ is the Hypergeometric Distribution.

%    
%    Let 
%    \begin{align*}
%        S_{even}&=\sum_{i \text{ even},0\leq i\leq k}\binom{k}{i}\binom{n-k}{|d|-i},\\
%        S_{odd}&=\sum_{i \text{ odd},0\leq i\leq k}\binom{k}{i}\binom{n-k}{|d|-i}.
%    \end{align*}
%    Then $S_{even}+S_{odd}=\binom{n}{|d|}$.
%    If $k$ is odd,  we have for even $i$
%    $$\frac{\binom{k}{i}\binom{n-k}{|d|-i}}{\binom{k}{i+1}\binom{n-k}{|d|-i-1}}=\frac{(i+1)(n-k-|d|+i+1)}{(k-i)(|d|-i)}\leq \frac{k(n-|d|)}{|d|-k+1}.$$
%    This means $S_{odd}\geq \frac{|d|-k+1}{k(n-|d|)}S_{even}$. Then 
%    $$P[x\cdot d=0]\leq \frac{1}{1+\frac{|d|-k+1}{k(n-|d|)}}<\frac{1}{1+\frac{1}{2k(k-1)}}<1-\frac{1}{4k(k-1)}.$$
%    The second inequality is by replacing $|d| $with $\frac{n}{k}$ and assuming $k^2<\frac{n}{2}$.\wxnote{This bound is not enough. can we do a finer analysis? How about calculating the generation function of hypergeometric distribution? The name of PGF of hypergeometric distribution is the gaussian hypergeometric function. 
%    Besides, I did some simple experiences for the value $\frac{S_{even}}{\binom{n}{|d|}}$ in which I chose $n=1000$, $k=32,31$, $d\in [1000]$. The value is almost symmetric as $d$ goes from 0 to 1000 for even $k$. For odd $k$, the value is decreasing with $d$.}
%
%    If $k$ is even, let $S'_{even}=S_{even}-\binom{n-k}{|d|-k}$. Since here $d$ is large, we can assume it is close to $\binom{n}{|d|}$ with a constant factor?
%
%    $S'_{even}+S_{odd}+\binom{n-k}{|d|-k}=\binom{n}{|d|}$.
%    Here $$(\frac{|d|}{n})^k>\frac{\binom{n-k}{|d|-k}}{\binom{n}{|d|}}=\frac{|d|\cdot (|d|-1)\cdot...\cdot(|d|-k)}{n\cdot ...\cdot (n-k) }\geq (\frac{|d|-k}{n-k})^k>(\frac{n/k-k}{n-k})^k>\frac{1}{(2k)^k}.$$
%    Thus $S'_{even}+S_{odd}=\binom{n}{|d|}-\binom{n-k}{|d|-k}<(1-\frac{1}{(2k)^k})\binom{n}{|d|}.$
%    A similar argument shows that $S_{odd}\geq \frac{|d|-k+1}{k(n-|d|)}S'_{even}$. Then  
%    $P[x\cdot d =0]<\frac{(1-(\frac{|d|-k}{n-k})^k)}{1+\frac{1}{2k(k-1)}}+(\frac{|d|}{n})^k<1-\frac{1}{8k(k-1)}.$ Here we assume $|d|<\frac{n}{1.01}.$ However for $d$ close to $n$, we can not use this trivial upper bound.
%    
\end{itemize}
\end{proofof}
\fi
